A Turkish Educational Crossword Puzzle Generator

This paper introduces the first Turkish crossword puzzle generator designed to leverage the capabilities of large language models (LLMs) for educational purposes. In this work, we introduced two specially created datasets: one with over 180,000 unique answer-clue pairs for generating relevant clues from the given answer, and another with over 35,000 samples containing text, answer, category, and clue data, aimed at producing clues for specific texts and keywords within certain categories. Beyond entertainment, this generator emerges as an interactive educational tool that enhances memory, vocabulary, and problem-solving skills. It's a notable step in AI-enhanced education, merging game-like engagement with learning for Turkish and setting new standards for interactive, intelligent learning tools in Turkish.

==> bib.tex <==
@article{orawiwatnakul2013crossword,
  title={Crossword puzzles as a learning tool for vocabulary development},
  author={Orawiwatnakul, Wiwat},
  journal={Electronic Journal of Research in Education Psychology},
  volume={11},
  number={30},
  pages={413--428},
  year={2013}
}


@article{bella2023improving,
  title={The Improving of the Student’s Vocabulary Achievement through Crossword Game in the New Normal Era},
  author={Bella, Yolanda Dita and Rahayu, Endang Mastuti},
  journal={Edunesia: Jurnal Ilmiah Pendidikan},
  volume={4},
  number={2},
  pages={830--842},
  year={2023}
}

@article{dzulfikri2016application,
  title={Application-Based Crossword Puzzles: Players’ Perception and Vocabulary Retention},
  author={Dzulfikri, Dzulfikri},
  journal={Studies in English Language and Education},
  volume={3},
  number={2},
  pages={122--133},
  year={2016}
}


@incollection{nickerson1977crossword,
  title={Crossword puzzles and lexical memory},
  author={Nickerson, RS},
  booktitle={Attention and performance VI},
  pages={699--718},
  year={1977},
  publisher={Routledge}
}

@article{yuriev2016crossword,
  title={Crossword puzzles for chemistry education: learning goals beyond vocabulary},
  author={Yuriev, Elizabeth and Capuano, Ben and Short, Jennifer L},
  journal={Chemistry education research and practice},
  volume={17},
  number={3},
  pages={532--554},
  year={2016},
  publisher={Royal Society of Chemistry}
}

@article{sandiuc2020use,
  title={The use of crossword puzzles as a strategy to teach Maritime English Vocabulary},
  author={Sandiuc, Corina and Balagiu, Alina},
  journal={Scientific Bulletin" Mircea cel Batran" Naval Academy},
  volume={23},
  number={1},
  pages={236A--242},
  year={2020},
  publisher={Naval Academy Publishing House}
}

@article{kaynak2023effect,
  title={The effect of crossword puzzle activity used in distance education on nursing students’ problem-solving and clinical decision-making skills: A comparative study},
  author={Kaynak, Serap and Erg{\"u}n, Sibel and Karada{\c{s}}, Ay{\c{s}}e},
  journal={Nurse Education in Practice},
  volume={69},
  pages={103618},
  year={2023},
  publisher={Elsevier}
}

@article{dzulfikri2016application,
  title={Application-Based Crossword Puzzles: Players’ Perception and Vocabulary Retention},
  author={Dzulfikri, Dzulfikri},
  journal={Studies in English Language and Education},
  volume={3},
  number={2},
  pages={122--133},
  year={2016}
}

@inproceedings{mueller2018testing,
  title={Testing the effectiveness of crossword games on immediate and delayed memory for scientific vocabulary and concepts.},
  author={Mueller, Shane T and Veinott, Elizabeth S},
  booktitle={CogSci},
  year={2018}
}


@article{zirawaga2017gaming,
  title={Gaming in education: Using games as a support tool to teach history.},
  author={Zirawaga, Victor Samuel and Olusanya, Adeleye Idowu and Maduku, Tinovimbanashe},
  journal={Journal of Education and Practice},
  volume={8},
  number={15},
  pages={55--64},
  year={2017},
  publisher={ERIC}
}

@article{bella2023improving,
  title={The Improving of the Student’s Vocabulary Achievement through Crossword Game in the New Normal Era},
  author={Bella, Yolanda Dita and Rahayu, Endang Mastuti},
  journal={Edunesia: Jurnal Ilmiah Pendidikan},
  volume={4},
  number={2},
  pages={830--842},
  year={2023}
}

@article{zamani2021use,
  title={The use of crossword puzzles as an educational tool},
  author={Zamani, Peyman and Haghighi, Somayeh Biparva and Ravanbakhsh, Majid},
  journal={Journal of Advances in Medical Education \& Professionalism},
  volume={9},
  number={2},
  pages={102},
  year={2021},
  publisher={Shiraz University of Medical Sciences}
}

@article{dol2017gpbl,
  title={GPBL: An effective way to improve critical thinking and problem solving skills in engineering education},
  author={Dol, Sunita M},
  journal={J Engin Educ Trans},
  volume={30},
  number={3},
  pages={103--13},
  year={2017}
}

@article{yuriev2016crossword,
  title={Crossword puzzles for chemistry education: learning goals beyond vocabulary},
  author={Yuriev, Elizabeth and Capuano, Ben and Short, Jennifer L},
  journal={Chemistry education research and practice},
  volume={17},
  number={3},
  pages={532--554},
  year={2016},
  publisher={Royal Society of Chemistry}
}

@inproceedings{rigutini2008fully,
  title={A fully automatic crossword generator},
  author={Rigutini, Leonardo and Diligenti, Michelangelo and Maggini, Marco and Gori, Marco},
  booktitle={2008 Seventh International Conference on Machine Learning and Applications},
  pages={362--367},
  year={2008},
  organization={IEEE}
}

@article{rigutini2012automatic,
  title={Automatic generation of crossword puzzles},
  author={Rigutini, Leonardo and Diligenti, Michelangelo and Maggini, Marco and Gori, Marco},
  journal={International Journal on Artificial Intelligence Tools},
  volume={21},
  number={03},
  pages={1250014},
  year={2012},
  publisher={World Scientific}
}

@inproceedings{ranaivo2013automatic,
  title={Automatic generation of fill-in clues and answers from raw texts for crosswords},
  author={Ranaivo-Malan{\c{c}}on, Bali and Lim, Terrin and Minoi, Jacey-Lynn and Jupit, Amelia Jati Robert},
  booktitle={2013 8th International Conference on Information Technology in Asia (CITA)},
  pages={1--5},
  year={2013},
  organization={IEEE}
}

@article{esteche2017automatic,
  title={Automatic Definition Extraction and Crossword Generation From Spanish News Text},
  author={Esteche, Jennifer and Romero, Romina and Chiruzzo, Luis and Ros{\'a}, Aiala},
  journal={CLEI Electronic Journal},
  volume={20},
  number={2},
  year={2017}
}

@inproceedings{arora2019automatic,
  title={Automatic keyword extraction and crossword generation tool for Indian languages: SEEKH},
  author={Arora, Bhavna and Kumar, NS},
  booktitle={2019 IEEE Tenth International Conference on Technology for Education (T4E)},
  pages={272--273},
  year={2019},
  organization={IEEE}
}


@inproceedings{zeinalipour2023arabicros,
  title={ArabIcros: AI-Powered Arabic Crossword Puzzle Generation for Educational Applications},
  author={Zeinalipour, Kamyar and Saad, Mohamed and Maggini, Marco and Gori, Marco},
  booktitle={Proceedings of ArabicNLP 2023},
  pages={288--301},
  year={2023}
}

@article{zeinalipour2023italian,
  title={Italian Crossword Generator: Enhancing Education through Interactive Word Puzzles},
  author={Zeinalipour, Kamyar and Zanollo, Asya and Angelini, Giovanni and Rigutini, Leonardo and Maggini, Marco and Gori, Marco and others},
  journal={arXiv preprint arXiv:2311.15723},
  year={2023}
}

@article{wang2022self,
  title={Self-instruct: Aligning language model with self generated instructions},
  author={Wang, Yizhong and Kordi, Yeganeh and Mishra, Swaroop and Liu, Alisa and Smith, Noah A and Khashabi, Daniel and Hajishirzi, Hannaneh},
  journal={arXiv preprint arXiv:2212.10560},
  year={2022}
}

